Chebyshev polynomials corresponding to a vanishing weight

We consider weighted Chebyshev polynomials on the unit circle corresponding to a weight of the form $(z-1)^s$ where $s>0$. For integer values of $s$ this corresponds to prescribing a zero of the polynomial on the boundary. As such, we extend findings of Lachance, Saff and Varga, to non-integer $s$. Using this generalisation, we are able to relate Chebyshev polynomials on lemniscates and other, more established, categories of Chebyshev polynomials. An essential part of our proof involves the broadening of the Erd\H{o}s--Lax inequality to encompass powers of polynomials. We believe that this particular result holds significance in its own right.

==> some_extra_results.tex <==
\begin{lemma}
            Let $p$ be a polynomial of degree $n$ with zeros $\left\{ c_{k} \right\}$ all in $\overline{\mathbb{D}}$ and $t_{k}(z) = \Im(z/(z-c_{k}))$, then
            \begin{equation*}
                \left\lvert \frac{p'(z)}{p(z)} \right\rvert^{2} \geq \frac{n^{2}}{4} + \left( \sum t_{k}(z) \right)^{2}, z \in \mathbb{T}.
            \end{equation*}
            \begin{proof}
                For $\lvert z \rvert = 1$,
                \begin{equation*}
                    \Re \left( \frac{z}{z-c_{k}} \right) = \frac{1}{2} \frac{2-2\Re(\overline{c_{k}}z)}{\lvert z - c_{k} \rvert^{2}} \geq \frac{1}{2}.
                \end{equation*}
                The result follows.
            \end{proof}
        \end{lemma}
        \begin{lemma}
            Let $f$ be as in \eqref{eq:form}, then for sufficiently large $M > 0$
            \begin{equation*}
                \int \log^{+} \left( M \frac{m}{n} \lvert f'(z) \rvert \right) dm \leq \int \log^{+} \lvert Mf(z) \rvert dm.
            \end{equation*}
            \begin{proof}
                The inequality is clear if $f$ has no zeros on the boundary, hence we will assume at least one $c_{k}$ is unimodular. Define two sets $E$ and $F$ by
                \begin{equation*}
                    E = \left\{ z \in \mathbb{T}: \frac{m}{n}\lvert f'(z) \rvert \leq 1 \right\},
                \end{equation*}
                and
                \begin{equation*}
                    F = \left\{ z \in \mathbb{T} : \lvert f(z) \rvert \leq 1 \right\}.
                \end{equation*}
                By the previous Lemma
                \begin{equation}\label{eq:est1}
                    \frac{m}{n}\lvert f'(z) \rvert = \lvert f(z) \rvert \frac{1}{n} \left\lvert \frac{p'(z)}{p(z)}\right\rvert \geq \lvert f(z) \rvert \left( \frac{1}{4} + \frac{1}{n^{2}} \left(\sum t_{k}(z) \right)^{2}\right)^{1/2}.
                \end{equation}
                Also
                \begin{equation}\label{eq:est2}
                    \int_{E} \log \lvert f(z) \rvert \geq \int_{F} \log \lvert f(z) \rvert.
                \end{equation}
                Combining \eqref{eq:est1} and \eqref{eq:est2} give
                \begin{equation*}
                    \begin{split}
                        \int_{E} \log \left\lvert \frac{m}{n} f'(z)\right\rvert = \int_{E} \log \left\lvert \frac{1}{n}f(z)\frac{p'(z)}{p(z)} \right\rvert \geq \int_{E} \log \left( \left\lvert f(z) \right\rvert \left( \frac{1}{4} + \frac{1}{n^{2}} \left(\sum t_{k}(z) \right)^{2}\right)^{1/2} \right) \\ = \int_{E} \log \lvert f(z) \rvert + \frac{1}{2}\log \left( \frac{1}{4} + \frac{1}{n^{2}} \left(\sum t_{k}(z) \right)^{2}\right) = \int_{E} \log \lvert f(z)/2 \rvert + \log \left(1 + 4\frac{1}{n^{2}} \left(\sum t_{k}(z) \right)^{2}\right)^{1/2} \\ \geq \int_{F} \log \left\lvert f(z) \right\rvert - \lvert E \rvert \log(2) + \int_{E} \log \left(1 + 4\frac{1}{n^{2}} \left(\sum t_{k}(z) \right)^{2}\right)^{1/2}.
                    \end{split}
                \end{equation*}
                Thus we have
                \begin{equation*}
                    \begin{split}
                        \int \log^{+}\left\lvert \frac{m}{n} f'(z)\right\rvert = \int \log \left\lvert \frac{m}{n} f'(z)\right\rvert - \int_{E} \log \left\lvert \frac{m}{n} f'(z)\right\rvert = \int \log \left\lvert f(z)\right\rvert - \int_{E} \log \left\lvert \frac{m}{n} f'(z)\right\rvert \\ \leq \int \log^{+} \left\lvert f(z)\right\rvert + \lvert E \rvert \log 2 - \int_{E} \log \left(1 + 4\frac{1}{n^{2}} \left(\sum t_{k}(z) \right)^{2}\right)^{1/2}.
                    \end{split}
                \end{equation*}
                Scaling $f$ by $M > 0$ we obtain
                \begin{equation*}
                    \int \log^{+}\left\lvert M \frac{m}{n} f'(z)\right\rvert \leq \int \log^{+} \left\lvert f(z)\right\rvert + \lvert E_{M} \rvert \log 2 - \int_{E_{M}} \log \left(1 + 4\frac{1}{n^{2}} \left(\sum t_{k}(z) \right)^{2}\right)^{1/2},
                \end{equation*}
                where $E_{M} = \left\{ M^{-1} \geq \frac{m}{n}\lvert f'(z) \rvert \right\}$. Thus to obtain the desired inequality we need to show that we can choose $M > 0$, such that
                \begin{equation*}
                    \int_{E_{M}} \log \left(1 + 4\frac{1}{n^{2}} \left(\sum t_{k}(z) \right)^{2}\right)^{1/2} \geq \lvert E_{M} \rvert \log(2).
                \end{equation*}
                Since $E_{M} \subset F_{M/2} = \left\{ M^{-1} \geq \lvert f(z) \rvert/2 \right\}$ (this follows from the inequality $m/n\lvert f' \rvert = n\lvert fp/p' \rvert \geq \lvert f \rvert/2$) it is sufficient to choose $M > 0$, such that
                \begin{equation*}
                    \left\lvert \sum t_{k}(z) \right\rvert \geq \frac{\sqrt{3}}{2}n \text{, for all } z \in F_{M/2},    
                \end{equation*}
                But this is possible since the $\sum t_{k}$ and $n$ are fixed and by increasing $M$ we get closer to the singularities of $\sum t_{k}(z)$ (recall that we have assumed at least one $c_{k}$ lies on the unit circle and so $\sum t_{k}$ has at least one singularity). \end{proof}
            \end{lemma}
            We are now ready to prove the Bernstein-type estimate (Actually we prove something stronger).


    \begin{section}{A Bernstein estimate}
        We begin by proving the "Bernstein type" estimate. We recall Mahler's inequality.
        \begin{lemma}
            Let $P$ be a polynomial of degree $n$, then
            \begin{equation*}
                \int_{0}^{2\pi} \log \lvert P'(e^{i\theta})/n \rvert \frac{d\theta}{2\pi} \leq \int_{0}^{2\pi} \log \lvert P(e^{i\theta}) \rvert\frac{d\theta}{2\pi}.
            \end{equation*}
            \begin{proof}
                It follows from Jensen's formula and the Gauss-Lucas Theorem that when $P$ has all of its zeros in $\overline{\mathbb{D}}$ the inequality is actually an equality. Otherwise let
                \begin{equation*}
                    P(z) = \prod_{k} (z-c_{k}),
                \end{equation*}
                and define a new polynomial $Q$ by
                \begin{equation*}
                    Q(z) = \left( \prod_{\lvert c_{k} \rvert \leq 1} (z-c_{k}) \right)\left( \prod_{\lvert c_{k} \rvert > 1} (1-\overline{c_{k}}z) \right).
                \end{equation*}
                Then $\lvert P(z) \rvert = \lvert Q(z) \rvert$ and $\lvert P'(z) \rvert \leq \lvert Q'(z) \rvert$, for $z \in \mathbb{T}$. Thus
                \begin{equation*}
                    \int_{0}^{2\pi} \log \lvert P'(e^{i\theta})/n \rvert \frac{d\theta}{2\pi}\leq \int_{0}^{2\pi} \log \lvert Q'(e^{i\theta})/n \rvert \frac{d\theta}{2\pi}= \int_{0}^{2\pi} \log \lvert Q(e^{i\theta}) \rvert\frac{d\theta}{2\pi} = \int_{0}^{2\pi} \log \lvert P(e^{i\theta}) \rvert\frac{d\theta}{2\pi}.
                \end{equation*}
            \end{proof}
        \end{lemma}
        We shall lift this to an inequality for $f$ in a series of lemmas.
        \begin{lemma}\label{lemma:log+}
            Let $s \in \mathbb{C}$ and $\zeta \in \mathbb{T}$, then
            \begin{equation*}
                \log^{+}\lvert s \rvert = \int \log \lvert s + \lambda \zeta \rvert dm(\lambda).
            \end{equation*}
            \begin{proof}
                If $\lvert s \rvert > 1$, then $\lambda \mapsto \log \lvert s + \lambda \zeta \rvert$ is harmonic in the unit disc and hence the formula is correct in this case. On the other hand if $\lvert s \rvert \leq 1$, then $\lambda \mapsto \log \lvert \lambda \zeta \overline{s} + 1\rvert$ is harmonic in the unit disc and hence the result follows.
            \end{proof}
        \end{lemma}
        \begin{lemma}\label{lemma:key_est}
            Let $f$ be as in \eqref{eq:form} with $s_{k} > 0$, then
            \begin{equation*}
                \int_{0}^{2\pi} \log^{+} \left( \frac{m}{n} \lvert P(e^{i\theta})f'(e^{i\theta}) \rvert\right)\frac{d\theta}{2\pi} \leq \int_{0}^{2\pi} \log^{+} \lvert P(e^{i\theta})f(e^{i\theta}) \rvert \frac{d\theta}{2\pi}. 
            \end{equation*}
            \begin{proof}
                Fix $\lvert \lambda \rvert = 1$. Applying Mahler's inequality the polynomial $Q_{\lambda}(z) = P(z) + z^{n}\lambda$ we obtain
                \begin{align*}
                \begin{split}
                    \frac{1}{m}\int_{0}^{2\pi} \log \lvert P(e^{i\theta}) + e^{in\theta}\lambda \rvert \frac{d\theta}{2\pi} + \int_{0}^{2\pi} \log \lvert P'(e^{i\theta})/n + e^{i(n-1)\theta}\lambda \rvert \frac{d\theta}{2\pi}\\ \leq \left(\frac{1}{m} + 1\right)\int_{0}^{2\pi} \log \lvert P(e^{i\theta}) + e^{in\theta}\lambda \rvert \frac{d\theta}{2\pi}.
                \end{split}
                \end{align*}
                Integrating in $\lambda$ and using Lemma \ref{lemma:log+} we obtain
                \begin{equation*}
                    \frac{1}{m}\int_{0}^{2\pi} \log^{+} \lvert P(e^{i\theta}) \rvert \frac{d\theta}{2\pi} + \int_{0}^{2\pi} \log^{+} \lvert P'(e^{i\theta})/n \rvert \frac{d\theta}{2\pi} \leq \left(\frac{1}{m} + 1\right)\int_{0}^{2\pi} \log^{+} \lvert P(e^{i\theta}) \rvert \frac{d\theta}{2\pi}.
                \end{equation*}
                using that $\log^{+}(a) + \log^{+}(b) \geq \log^{+}(ab)$ we obtain
                \begin{align*}
                    \begin{split}
                        \int_{0}^{2\pi} \log^{+} \lvert f(e^{i\theta})P(e^{i\theta}) \rvert \frac{d\theta}{2\pi}&=\int_{0}^{2\pi}\log^{+}|f(e^{i\theta})|\frac{d\theta}{2\pi}+\int_{0}^{2\pi}\log^{+}|P(e^{i\theta})|\frac{d\theta}{2\pi}\\&\geq \int_{0}^{2\pi}\log^{+}|f(e^{i\theta})|\frac{d\theta}{2\pi}+\int_{0}^{2\pi}\log^{+}|P'(e^{i\theta})/n|\frac{d\theta}{2\pi} \\ &= \int_{0}^{2\pi} \log^{+} \lvert f(e^{i\theta})P'(e^{i\theta})/n \rvert \frac{d\theta}{2\pi}\\& = \int_{0}^{2\pi} \log^{+} \left( \frac{m}{n} \lvert P(e^{i\theta})f'(e^{i\theta}) \rvert \right)\frac{d\theta}{2\pi}.    
                    \end{split}
                \end{align*}
            \end{proof}
        \end{lemma}
        \begin{lemma}
            Let $f$ be as in \eqref{eq:form}, then
            \begin{equation*}
                \norm{Pf'}_{p} \leq \frac{n}{m}\norm{Pf}_{p} \text{, for all } 0 \leq p \leq \infty.
            \end{equation*}
            \begin{proof}
                For $s \geq 0$ and $0 < p < \infty$
                \begin{equation*}
                    s^{p} = p^{2}\int_{0}^{\infty} t^{p-1}\log^{+}(s/t) dt.
                \end{equation*}
                Using this identity and Lemma \ref{lemma:key_est} to compute the $p$ norm of $Pf'$ gives
                \begin{equation*}
                \begin{split}
                    \int_{0}^{2\pi} \lvert \frac{m}{n} P(e^{i\theta})f'(e^{i\theta}) \rvert^{p} \frac{d\theta}{2\pi} = \int_{0}^{2\pi} p^{2}\int_{0}^{\infty} t^{p-1}\log^{+}\left(\frac{m\lvert P(e^{i\theta})f'(e^{i\theta}) \rvert}{nt}\right) dt \frac{d\theta}{2\pi} \\ \leq \int_{0}^{2\pi} p^{2}\int_{0}^{\infty} t^{p-1}\log^{+}\left(\frac{\lvert P(e^{i\theta})f(e^{i\theta}) \rvert}{t}\right) dt \frac{d\theta}{2\pi} = \int_{0}^{2\pi} \lvert \frac{m}{n} P(e^{i\theta})f(e^{i\theta})\rvert^{p} \frac{d\theta}{2\pi}. 
                \end{split}
                \end{equation*}
            \end{proof}
        \end{lemma}
        Now it would be interesting to show that in the case $s_{k} \geq 1$ we can replace the above inequality with $\norm{f'}_{p} \leq \frac{n}{m}\norm{f}_{p}$. \newline
        
        Finally, we consider $f$ with zeros only on the unit circle and remark that the reverse inequality $\norm{f'}_{p} \geq \frac{n}{2m} \norm{f}_{p}$ is also valid for all $0 \leq p \leq \infty$. Thus we have (if the above guess is correct)
        \begin{equation*}
            \frac{n}{2m} \norm{f}_{p} \leq \norm{f'}_{p} \leq \frac{n}{m} \norm{f}_{p} \text{, for all } 0 \leq p \leq \infty.
        \end{equation*}
        It is interesting to note that the right inequality is sharp for $p = 0$ and the left for $p = \infty$ (as to be seen in the next section!). It seems to be an interesting problem to determine the sharp constants for all $0 < p < \infty$. Here the $p = 0$ norm is
        \begin{equation*}
            \norm{f}_{0} = \exp \left( \int \log \lvert f \rvert dm \right).
        \end{equation*}
        From analogy with the case of polynomials it seems that the optimal constant should be
        \begin{equation*}
            \norm{f'}_{p} \leq C(p)\frac{n}{m} \norm{f}_{p} \text{, for all } 0 \leq p \leq \infty,
        \end{equation*}
        with
        \begin{equation*}
            C(p) = \norm{1+z^{n}}_{p}^{-1}.
        \end{equation*}
        This is the case for polynomials as shown by Lax ($p = \infty$, $p = 2$), Zygmund ($p \geq 1$), and Arestov $0 < p < 1$.
    \end{section}

    @article{Lax,
author = {P. Lax},
title = {{Proof of a conjecture of P. Erd\H{o}s on the derivative of a polynomial}},
volume = {50},
journal = {Bulletin of the American Mathematical Society},
number = {8},
publisher = {American Mathematical Society},
pages = {509 -- 513},
year = {1944},
}
@article{ChristiansenRubin,
author = {Christiansen, J. S.
         and Rubin, O.},
title = {Chebyshev polynomials on lemniscates },
journal = {to appear},
year = {2023}
}

@article{LachanceSaffVarga,
author={Lachance, M.
and Saff, E. B.
and Varga, R. S.},
title={Inequalities for polynomials with a prescribed zero},
journal={Mathematische Zeitschrift},
year={1979},
month={Jun},
day={01},
volume={168},
number={2},
pages={105-116},
issn={1432-1823},
}

@article{AzizMohammad,
 ISSN = {00029939, 10886826},
 abstract = {An elementary new and simple proof of Erd\H{o}s-Lax theorem is given which in essence involves no analysis.},
 author = {A. Aziz and Q. G. Mohammad},
 journal = {Proceedings of the American Mathematical Society},
 number = {1},
 pages = {119--122},
 publisher = {American Mathematical Society},
 title = {Simple Proof of a Theorem of {E}rd{\H o}s and {L}ax},
 volume = {80},
 year = {1980}
}
@article{MirHussainWagay,
author={Mir, A.
and Hussain, A.
and Wagay, F. A.},
title={On the Erd{\"o}s-Lax inequality and its various generalizations concerning polynomials},
journal={Rendiconti del Circolo Matematico di Palermo Series 2},
year={2023},
month={Apr},
day={01},
volume={72},
number={3},
pages={2025-2037},
issn={1973-4409},
}

@article{Malik,
    author = {M. A. Malik},
    title = "{On the Derivative of a Polynomial}",
    journal = {Journal of the London Mathematical Society},
    volume = {s2-1},
    number = {1},
    pages = {57-60},
    year = {1969},
    month = {01},
    issn = {0024-6107},
}



@article{Turan,
    author = {P. Tur\'{a}n'},
    title = {\"{u}ber die Ableitung von Polynomen},
    journal = {Compositio Math},
    volume = {7},
    pages = {89--95},
    year = {1939}
}

@article{RAHMAN198826,
title = {L$^p$ inequalities for polynomials},
journal = {Journal of Approximation Theory},
volume = {53},
number = {1},
pages = {26-32},
year = {1988},
issn = {0021-9045},
author = {Q.I Rahman and G Schmeisser}
}

@article{arestov1981integral,
  title={On integral inequalities for trigonometric polynomials and their derivatives},
  author={Arestov, Vitalii Vladimirovich},
  journal={Izvestiya Rossiiskoi Akademii Nauk. Seriya Matematicheskaya},
  volume={45},
  number={1},
  pages={3--22},
  year={1981},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian~…}
}

@article {MR0023380,
    AUTHOR = {de Bruijn, N. G.},
     TITLE = {Inequalities concerning polynomials in the complex domain},
   JOURNAL = {Nederl. Akad. Wetensch., Proc.},
  FJOURNAL = {Proceedings. Akadamie van Wetenschappen Amsterdam.
              North-Holland, Amsterdam},
    VOLUME = {50},
      YEAR = {1947},
     PAGES = {1265--1272 = Indagationes Math. {\bf 9, 591--598}},
      ISSN = {0370-0348},
   MRCLASS = {41.1X},
  MRNUMBER = {23380},
MRREVIEWER = {A.\ Zygmund},
}

@article {MR1576159,
    AUTHOR = {Zygmund, A.},
     TITLE = {A {R}emark on {C}onjugate {S}eries},
   JOURNAL = {Proc. London Math. Soc. (2)},
  FJOURNAL = {Proceedings of the London Mathematical Society. Second Series},
    VOLUME = {34},
      YEAR = {1932},
    NUMBER = {5},
     PAGES = {392--400},
      ISSN = {0024-6115},
   MRCLASS = {99-04},
  MRNUMBER = {1576159},
}
